Training and inference of large language models using 8-bit floating point

FP8 formats are gaining popularity to boost the computational efficiency for training and inference of large deep learning models. Their main challenge is that a careful choice of scaling is needed to prevent degradation due to the reduced dynamic range compared to higher-precision formats. Although there exists ample literature about selecting such scalings for INT formats, this critical aspect has yet to be addressed for FP8. This paper presents a methodology to select the scalings for FP8 linear layers, based on dynamically updating per-tensor scales for the weights, gradients and activations. We apply this methodology to train and validate large language models of the type of GPT and Llama 2 using FP8, for model sizes ranging from 111M to 70B. To facilitate the understanding of the FP8 dynamics, our results are accompanied by plots of the per-tensor scale distribution for weights, activations and gradients during both training and inference.

==> fig/inference_and_finetuning_validation_acc.tex <==
\begin{table}
\centering
\begin{tabular}{cc|ccc|ccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Quantisation}} & \multicolumn{3}{c|}{\textbf{Inference}} & \multicolumn{3}{c}{\textbf{Fine-tuning}} \\

& & MNLI & QQP & SST2 & MNLI & QQP & SST2 \\
\hline
\multirow{3}{*}{111M} & FP16       & 72.61 & 85.76 & 84.26 & 72.61 & 85.32 & 85.07 \\
                      & FP8-AMAX   & 72.39 & 85.78 & 84.38 & 72.50 & 85.84 & 85.57 \\
                      & FP8-CSCALE & 72.49 & 85.73 & 84.59 &  & & \\
\hline
\multirow{3}{*}{590M} & FP16       & 78.59 & 88.40 & 90.63 & 78.59 & 88.25 & 89.27 \\
                      & FP8-AMAX   & 78.44 & 88.37 & 90.63 & 79.12 & 88.31 & 89.00 \\
                      & FP8-CSCALE & 78.56 & 88.40 & 90.54 & & & \\
\hline
\multirow{3}{*}{1.3B} & FP16       & 82.82 & 89.43 & 91.55 & 82.82  & 89.32  & 91.36 \\
                      & FP8-AMAX   & 82.68 & 89.42 & 91.44 & 82.58  & 89.32  & 91.28 \\
                      & FP8-CSCALE & 82.72 & 89.36 & 91.42 &   &  &  \\
\hline
\multirow{3}{*}{6.7B} & FP16       & 87.17 & 91.19 & 94.50 & 87.17   & 91.19  & 94.53 \\
                      & FP8-AMAX   & 87.15 & 91.22 & 94.38 & 87.26   & 91.06  & 94.84 \\
                      & FP8-CSCALE & 87.18 & 91.18 & 94.48 &   &  &  \\
\hline
\multirow{3}{*}{13B}  & FP16       & 88.26 & TBD & 94.61 & 88.26   & TBD    & 94.61 \\
                      & FP8-AMAX   & 88.27 & TBD & 94.61 & TBD     & TBD    & 94.50 \\
                      & FP8-CSCALE & 88.26 & TBD & 94.50 &   &  &  \\
\hline
\vspace{0.05cm}
\end{tabular}
\caption{Comparison of validation accuracy for inference and fine-tuning, comparing FP16 with FP8-AMAX and FP8-CSCALE, for different model sizes ranging from 111M to 13B parameters. In the three tasks the validation metric is accuracy. The hyphen "-" denotes that convergence cannot be achieved for that task and model size with the FP8-CSCALE method.}
\label{tab:validation_gpt_models}


% \hspace{0.05\textwidth}%

% \begin{minipage}{.6\textwidth}
% \centering
% \begin{tabular}{ccccc}
% \hline
% \textbf{Model} & \textbf{Quantisation} &\textbf{MNLI} & \textbf{QQP} & \textbf{SST} \\
% \hline
% \multirow{3}{*}{111M} & FP16       & 72.61 & 85.32 & 85.07 \\
%                       & FP8-AMAX   & 72.50 & 85.84 & 85.57 \\
% \hline
% \multirow{3}{*}{590M} & FP16       & 78.59 & 88.25 & 89.27 \\
%                       & FP8-AMAX   & 79.12 & 88.31 & 89.00 \\
% \hline
% \multirow{3}{*}{1.3B} & FP16       & 82.82 & 89.32 & 91.36 \\
%                       & FP8-AMAX   & 82.58 & 89.32 & 91.28 \\
% \hline
% \multirow{3}{*}{6.7B} & FP16       & 87.17 & 91.19 & 94.53 \\
%                       & FP8-AMAX   & 87.26 & 91.06 & 94.84 \\
% \hline
% \multirow{3}{*}{13B}  & FP16       & 88.26 & TBD   & 94.61 \\
%                       & FP8-AMAX   & TBD   & TBD   & 94.50 \\
% \hline
% \vspace{0.05cm}
% \end{tabular}
% % \caption{\textbf{Fine-tuning results}: validation accuracy after fine-tuning in FP16 and FP8-AMAX for 3 epochs, for different model sizes ranging from 111M to 13B parameters. In the four tasks the validation metric is accuracy.}
% \label{tab:finetuning_gpt_models}
% \end{minipage}
\end{table}

==> fig/training_gpt_constant_scaling.tex <==

\begin{table}
\centering
\begin{tabular}{cc}
\hline
\textbf{Model} & \textbf{MNLI} \\
\hline
111M & [-3, 2] \\
590M & [-2, 2]  \\
1.3B and larger & Nil \\
\hline
\vspace{0.05cm}
\end{tabular}
\caption{Range of the scaling bias that doesn't degrade the accuracy by more than 0.5\% from the FP16 result when performing FP8 fine-tuning with constant scaling bias (FP8-CSCALE). Weights, activations and gradients in all decoders share the same scaling bias.}
\label{tab:fixed_scaling_bias_training}
\end{table}
